Terminal Brain Damage: Exposing the Graceless Degradation in Deep Neural Networks Under Hardware Fault Attacks

Deep neural networks (DNNs) have been shown to tolerate "brain damage": cumulative changes to the network's parameters (e.g., pruning, numerical perturbations) typically result in a graceful degradation of classification accuracy. However, the limits of this natural resilience are not well understood in the presence of small adversarial changes to the DNN parameters' underlying memory representation, such as bit-flips that may be induced by hardware fault attacks. We study the effects of bitwise corruptions on 19 DNN models---six architectures on three image classification tasks---and we show that most models have at least one parameter that, after a specific bit-flip in their bitwise representation, causes an accuracy loss of over 90%. We employ simple heuristics to efficiently identify the parameters likely to be vulnerable. We estimate that 40-50% of the parameters in a model might lead to an accuracy drop greater than 10% when individually subjected to such single-bit perturbations. To demonstrate how an adversary could take advantage of this vulnerability, we study the impact of an exemplary hardware fault attack, Rowhammer, on DNNs. Specifically, we show that a Rowhammer enabled attacker co-located in the same physical machine can inflict significant accuracy drops (up to 99%) even with single bit-flip corruptions and no knowledge of the model. Our results expose the limits of DNNs' resilience against parameter perturbations induced by real-world fault attacks. We conclude by discussing possible mitigations and future research directions towards fault attack-resilient DNNs.

==> figures/characterizations.tex <==


% multiple plots as the custom format
\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.29\textwidth]{figures/char_bitposition.pdf}
	\includegraphics[width=0.39\textwidth]{figures/char_bitdirections.pdf}
	\includegraphics[width=0.29\textwidth]{figures/char_dropbnorm.pdf}
	\includegraphics[width=0.46\textwidth]{figures/char_signs.pdf}
	\includegraphics[width=0.43\textwidth]{figures/char_activation.pdf}
	\caption{\textbf{Characterize the vulnerability.} We analyze the vulnerability based on the impact of: (a) the bit positions, (b) flip directions, (c) Dropout and batch normalization, (d) parameter signs, and (e) activation.}
	\label{fig:characterizations}
\end{figure*}

==> numbers.tex <==
%--------------------------------------------------------------------------
% Numbers that must be quoted consistently throughout the paper
\newcommand{\ApplicationsSelected}[0]{10\xspace}
\newcommand{\HostsWINEMillions}[0]{8.4\xspace}
\newcommand{\FilesWINE}[0]{7,196,952\xspace}
\newcommand{\FilesWINEMillions}[0]{7.1\xspace}
\newcommand{\ExploitsWINEAV}[0]{244\xspace}
\newcommand{\FilesVT}[0]{5,194,029\xspace}
\newcommand{\FilesVTMillions}[0]{5.1\xspace}
\newcommand{\NVDVuls}[0]{59,875\xspace}
\newcommand{\NVDVulsThousands}[0]{59\xspace}
\newcommand{\OSVDBVuls}[0]{77,101\xspace}
\newcommand{\OSVDBVulsThousands}[0]{77\xspace}
\newcommand{\EDBExploits}[0]{25,331\xspace}
\newcommand{\EDBExploitsThousands}[0]{25\xspace}
\newcommand{\VulnerabilitiesSelected}[0]{1,593\xspace}
\newcommand{\VulnerabilityClusters}[0]{408\xspace}		% only 397 in the survival data
\newcommand{\VulnerabilitiesPerCluster}[0]{3.9\xspace}
\newcommand{\ObservationPeriodLengthYears}[0]{5\xspace}


\newcommand{\SoPWeekBeforeAfter}[0]{77\%\xspace}
\newcommand{\SoPMonthBeforeAfter}[0]{92\%\xspace}
\newcommand{\MedianTimeToPatchVulnPrctReached}[0]{87\%\xspace}
\newcommand{\MedianTimeToPatchClustPrctReached}[0]{78\%\xspace}
\newcommand{\MedianTimeToPatchMin}[0]{0\xspace}
\newcommand{\MedianTimeToPatchMax}[0]{1156\xspace}
\newcommand{\MedianTimeToPatchMedian}[0]{45\xspace}
\newcommand{\MedianTimeToPatchAverage}[0]{101\xspace}
\newcommand{\NinetyfiveTimeToPatchVulnPrctReached}[0]{28\%\xspace}
\newcommand{\NinetyfiveTimeToPatchClustPrctReached}[0]{26\%\xspace}
\newcommand{\NinetyfiveTimeToPatchMin}[0]{0\xspace}
\newcommand{\NinetyfiveTimeToPatchMax}[0]{1452\xspace}
\newcommand{\NinetyfiveTimeToPatchMedian}[0]{429\xspace}
\newcommand{\NinetyfiveTimeToPatchAverage}[0]{434\xspace}
\newcommand{\ExploitsMatchedWINE}[0]{13\xspace}		% 11 distinct CVEs (some CVEs affect more than one app)
\newcommand{\ExploitsMatchedEDB}[0]{50\xspace}		% 46 distinct CVEs
\newcommand{\ExploitsMatchedAll}[0]{54\xspace}		% 50 distinct CVEs
\newcommand{\VulnerabilitySurvivalAtExploitationMedian}{86\%\xspace}
\newcommand{\PatchLevelAtExploitationMedian}{14\%\xspace}
\newcommand{\PatchCompletionCutoff}[0]{98.7\%\xspace}
\newcommand{\PatchCompletionVulnerabilities}[0]{30\xspace}
\newcommand{\PatchCompletionHalfTimeMeanClusters}[0]{213 days\xspace}  % 213.4749035
%--------------------------------------------------------------------------



==> tables/threat_model.tex <==


% - clarification of threat model: based on the attacker's capability
\begin{table}[h]
	\begin{tabular}{@{}lll@{}}
		\toprule
		Attacker's capability & Blind & Informed \\ \midrule
		Model knowledge &  &  \\
		&  &  \\ \bottomrule
	\end{tabular}
	\caption{}
	\label{tbl:threat-model}
\end{table}
